Downlink Performance of Superimposed Pilots in Massive MIMO systems

In this paper, we investigate the downlink throughput performance of a massive multiple-input multiple-output (MIMO) system that employs superimposed pilots for channel estimation. The component of downlink (DL) interference that results from transmitting data alongside pilots in the uplink (UL) is shown to decrease at a rate proportional to the square root of the number of antennas at the BS. The normalized mean-squared error (NMSE) of the channel estimate is compared with the Bayesian Cram\'{e}r-Rao lower bound that is derived for the system, and the former is also shown to diminish with increasing number of antennas at the base station (BS). Furthermore, we show that staggered pilots are a particular case of superimposed pilots and offer the downlink throughput of superimposed pilots while retaining the UL spectral and energy efficiency of regular pilots. We also extend the framework for designing a hybrid system, consisting of users that transmit either regular or superimposed pilots, to minimize both the UL and DL interference. The improved NMSE and DL rates of the channel estimator based on superimposed pilots are demonstrated by means of simulations.

==> texFiles/iterativeMethodDownlink.tex <==
\subsection{Downlink Performance With Iterative Data-Aided Channel Estimate}
\label{sec:dlSinrIterative}
% - Calculations for this section are in Book 3 dated 24/01/2018 - %
A simple iterative data-aided channel estimation method has been shown to reduce the UL interference resulting from transmitting the pilots alongside the data in \cite{upadhya2016superimposed}. In this subsection, we describe a majorization-minimization-based channel estimation algorithm to iteratively estimate the channel and UL data, and characterize its performance by means of simulations in Section \ref{sec:simulationResults}.

We assume for the remainder of this sub-section that the UL data is chosen from a finite constellation $ \dataConstellation $ with $ \constellationSize $ points.\footnote{ The assumption of a finite constellation has been made only for this subsection and does not influence the results obtained elsewhere in the manuscript.} Replacing the tuple $ \lrc{\sIdxOne,\sIdxTwo} $ with a single index $ \userIdx = 0,1,\ldots,N-1 $, where $ N \triangleq KL $, the received symbol vector at BS $ \vIdxOne $ in \eqref{eqn:ulSystemModel} can be rewritten as
\begin{align}
	\mbf{Y}
	=
	\mbf{H}
	\lrc{
		\rhoD{}{}
		\mbf{X}
		+
		\rhoP{}{}
		\mbf{P}
	}
	+
	\mbf{W}
\end{align}
where $ \mbf{H} = \lrs{\mbf{h}_{\vIdxOne0},\ldots\mbf{h}_{\vIdxOne,N-1}} \in \mathbb{C}^{M\times \pilotReuseRatioSp K} $, $ \mbf{X} = \lrs{\mbf{x}_0,\ldots,\mbf{x}_{N-1}}^T \in \mathbb{C}^{N\times \ulDuration}$, $ {\mbf{P} = \lrs{\spPilot{}{0},\ldots,\spPilot{}{N-1}}^T \in \mathbb{C}^{N\times \ulDuration}} $, and the subscript $ \vIdxOne $ has been dropped for notational convenience. In order to obtain an estimate of the channel and UL data, we obtain the estimates of $ \mbf{H} $ and $ \mbf{X} $ by solving the following optimization problem
\begin{align}
	\lrf{\widehat{\mbf{H}},\widehat{\mbf{X}}}
	&=
	\arg
	\max_{\mbf{H},\lrs{\mbf{X}}_{\elementIdxOne,\elementIdxTwo} \in \dataConstellation}
	\logLikelihood\lrc{\mbf{H},\mbf{X}}
	\label{eqn:llrMaximization}
\end{align}
where $ \logLikelihood\lrc{\mbf{H},\mbf{X}} $ is the log-likelihood ratio (LLR) and is defined as
\begin{align}
\logLikelihood\lrc{\mbf{H},\mbf{X}}
&\triangleq
	\log
	\lrs{p(\mbf{Y},\mbf{H}\;;\; \mbf{X})}
	=
	\lrf{
	\log
	\lrs{p(\mbf{Y}\condProb\mbf{H}\;;\; \mbf{X})}
	+
	\log
	\lrs{p(\mbf{H})}
	}
	\nonumber
	\\
	&\propto
	-
	\lrc{
	\left\| \mbf{Y} - \mbf{H}\lrc{\rhoD{}{}\mbf{X} + \rhoP{}{}\mbf{P}} \right\|^2_F
	+
	\sigma^2
	\mathrm{trace}
	\lrc{
		\mbf{H}
		\mbf{D}^{-1}
		\mbf{H}^H}
	}
	\label{eqn:llrDefn}
\end{align}
where $ \mbf{D} = \mathrm{diag}\lrf{\beta_{0},\ldots,\beta_{N-1}} $.

Since the optimization problem \eqref{eqn:llrMaximization} is non-convex in general, but concave in the individual variables $ \mbf{H} $ and $ \mbf{X} $, we maximize the LLR using alternating maximization. Given the $ \iterIdx\rth $ iterates of $ \mbf{H} $ and $ \mbf{X} $, the $ \iterIdx+1\rth $ iterate can be obtained as
\begin{align}
\mbf{X}^{(\iterIdx+1)} &= \arg\max_{\lrs{\mbf{X}}_{\elementIdxOne,\elementIdxTwo} \in \dataConstellation} \logLikelihood\lrc{\mbf{H}^{(\iterIdx)},\mbf{X}}
= 
\arg\min_{\lrs{\mbf{X}}_{\elementIdxOne,\elementIdxTwo}\in \dataConstellation}
\left\| \mbf{Y} - \mbf{H}^{(\iterIdx)}\lrc{\rhoD{}{}\mbf{X} + \rhoP{}{}\mbf{P}} \right\|^2_F
\label{eqn:xUpdate} \\ 
\mbf{H}^{(\iterIdx+1)} &= \arg\max_{\mbf{H}} \logLikelihood\lrc{\mbf{H},\mbf{X}^{(\iterIdx+1)}} 
= \arg \min_{\mbf{H}}
\left\| \mbf{Y} - \mbf{H}\lrc{\rhoD{}{}\mbf{X}^{(\iterIdx+1)} + \rhoP{}{}\mbf{P}} \right\|^2_F
\nonumber
\\
&
\qquad\qquad\qquad\qquad\qquad\qquad
+
\sigma^2
\mathrm{trace}
\lrc{
	\mbf{H}
	\mbf{D}^{-1}
	\mbf{H}^H}
\label{eqn:hUpdate} \;.
\end{align}
Defining $ \mbf{y}_{\symbolIdx} $, $ \mbf{x}_{\symbolIdx} $ and $ \mbf{p}_{\symbolIdx} $ to be the $ \symbolIdx\rth $ columns of $ \mbf{Y} $, $ \mbf{X} $, and $ \mbf{P} $, respectively, and $ \tilde{\mbf{y}}_{\symbolIdx} \triangleq \mbf{y}_{\symbolIdx} - \mbf{H}^{(\iterIdx)} \lrc{\rhoD{}{}\mbf{x}_{\symbolIdx}^{(\iterIdx)} +\rhoP{}{}\mbf{p}_{\symbolIdx}} $, the objective function in \eqref{eqn:xUpdate} can be written as
\begin{align}
&\left\| \mbf{Y} - \mbf{H}^{(\iterIdx)}\lrc{\rhoD{}{}\mbf{X} + \rhoP{}{}\mbf{P}} \right\|^2_F
=
\sum\limits_{\symbolIdx=0}^{\ulDuration-1}
\left\| 
\tilde{\mbf{y}}_{\symbolIdx}
- 
\rhoD{}{}\mbf{H}^{(\iterIdx)}\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}} 
\right\|^2
\nonumber
\\
&\!=\!\!
\sum\limits_{\symbolIdx=0}^{\ulDuration-1}
\!\!
\lrs{
	\|\tilde{\mbf{y}}_{\symbolIdx}\|^2
	\!
	+
	\!	
	\rhoD{}{}^2
	\!
	\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}}^{\!\!H}
	\!\!
	\lrc{\mbf{H}^{(\iterIdx)}}^{\!\!H}\!\!\mbf{H}^{(\iterIdx)}
	\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}}
	-
	2\rhoD{}{}\Re
	\lrf{
		\tilde{\mbf{y}}_{\symbolIdx}^H
		\mbf{H}^{(\iterIdx)}
		\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}}
		}
}\;.
\label{eqn:xOptimizationObjective}
\end{align}
Note that \eqref{eqn:xOptimizationObjective} is separable in $ \symbolIdx $ and therefore, each $ \mbf{x}_{\symbolIdx} $ can be optimized separately, i.e., 
\begin{align}
	\mbf{x}_{\symbolIdx}^{(i+1)}
	\!
	=
	\arg\min_{\lrs{\mbf{x}}_{\elementIdxOne}\in \dataConstellation}
		\rhoD{}{}^2
		\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}}^{\!\!H}
		\!\!
		\lrc{\!\mbf{H}^{(\iterIdx)}\!}^{\!\!H}\!\!\mbf{H}^{(\iterIdx)}
		\lrc{\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}}
		\!
		-
		2\rhoD{}{}\Re
		\lrf{
			\tilde{\mbf{y}}_{\symbolIdx}^H
			\mbf{H}^{(\iterIdx)}\!
			\lrc{\!\mbf{x}_{\symbolIdx} - \mbf{x}_{\symbolIdx}^{(\iterIdx)}\!}
		\!}\;.
	\label{eqn:xOptimizationSeparatedObjective}
\end{align} 
However, since each element of $ \mbf{x}_{\symbolIdx} $ can take $ \constellationSize $ values and since the first term in \eqref{eqn:xOptimizationSeparatedObjective} results in the optimization variables being coupled with each other, solving \eqref{eqn:xOptimizationSeparatedObjective} requires evaluating the objective function over $ \constellationSize^N $ points. Therefore, the complexity of \eqref{eqn:xOptimizationSeparatedObjective} increases exponentially in $ N $. 

To decouple the optimization problem, we employ a Gauss-Seidel-type method wherein each element of $ \mbf{x}_{\symbolIdx} $ is cyclically optimized by fixing the other elements to their latest estimates. Dropping the subscript $ \symbolIdx $ for notational convenience and using $ \lrs{z;\mbf{x}_{-\userIdx}^{(i)}} $ to denote $ \lrs{\lrs{\mbf{x}^{(\iterIdx+1)}}_{0}, \ldots, \lrs{\mbf{x}^{(\iterIdx+1)}}_{\userIdx-1} , z , \lrs{\mbf{x}^{(\iterIdx)}}_{\userIdx+1} ,\ldots, \lrs{\mbf{x}^{(\iterIdx)}}_{N-1} }^T$, $ \lrs{\mbf{x}^{(i+1)}}_{\userIdx} $ is obtained by setting $ \mbf{x}_{\symbolIdx} $ in \eqref{eqn:xOptimizationSeparatedObjective} to $ \lrs{x;\mbf{x}_{-\userIdx}^{(i)}} $, which results in the following optimization problem.
\begin{align}
\lrs{\mbf{x}^{(i+1)}}_{\userIdx}
=
\arg\min_{x \in \dataConstellation}
\rhoD{}{}^2
\left\|\mbf{h}^{(\iterIdx)}_{\userIdx}\right\|^2
\left|x - \lrs{\mbf{x}^{(\iterIdx)}}_{\userIdx}\right|^2
-
2\rhoD{}{}\Re
\lrf{
	\tilde{\mbf{y}}_{\userIdx}^H
	\mbf{h}^{(\iterIdx)}_{\userIdx}
	\lrc{x - \lrs{\mbf{x}^{(\iterIdx)}}_{\userIdx}}
	\!}
\label{eqn:xOptimizationPerElement}
\end{align} 
where $ \tilde{\mbf{y}}_{\userIdx} \triangleq \mbf{y} - \mbf{H}^{(\iterIdx)}\lrc{\rhoD{}{} \lrs{\lrs{x^{(\iterIdx)}}_{\userIdx};\mbf{x}_{-\userIdx}^{(i)}} + \rhoP{}{} \mbf{p}} $.

Using the estimate in the $ \iterIdx+1\rth $ iteration $ \mbf{H}^{(\iterIdx+1)} $ can be obtained from \eqref{eqn:hUpdate} as
\begin{align}
	\mbf{H}^{(\iterIdx+1)}
	=
	\mbf{Y}
	\lrc{\rhoD{}{}\mbf{X}^{(\iterIdx+1)} + \rhoP{}{}\mbf{P}}^H
	\lrc{\lrc{\rhoD{}{}\mbf{X}^{(\iterIdx+1)} + \rhoP{}{}\mbf{P}}^H\lrc{\rhoD{}{}\mbf{X}^{(\iterIdx+1)} + \rhoP{}{}\mbf{P}} + \sigma^2\mbf{D}^{-1}}^{-1}\;.
	\label{eqn:hOptimization}
\end{align}
It is straightforward to show that \eqref{eqn:xOptimizationPerElement} and \eqref{eqn:hOptimization} result in $ \logLikelihood\lrc{\mbf{H}^{(\iterIdx+1)},\mbf{X}^{(\iterIdx+1)}} \geq \logLikelihood\lrc{\mbf{H}^{(\iterIdx)},\mbf{X}^{(\iterIdx)}} $ in each iteration, and therefore, the aforementioned approach converges.

\begin{remark}
	Since \eqref{eqn:xOptimizationSeparatedObjective} is non-convex, the solution to the optimization problem also depends on the order in which the Gauss-Seidel-type iterations are executed. We order the interfering users such that $ \beta_{\userIdx} \geq \beta_{\vIdxTwo} $ when $ \userIdx<\vIdxTwo $, and the iterations proceed with increasing $ \userIdx $. This ordering ensures that the UL data of stronger interfering users are estimated first.
\end{remark}

\begin{remark}
	Note that iterative data-aided methods that maximize the LLR of the channel and/or UL data are not suitable when the UL symbols $ \lrs{\mbf{x}}_{\symbolIdx} $ are continuous random variables, such as in the case of a Gaussian constellation. This is because, in the absence of constraints on the UL data, an iterative algorithm can choose $ \lrs{\widehat{\mbf{x}}}_{\symbolIdx} $ to maximize the LLR by penalizing the MSE of $ \widehat{\mbf{h}}_{\userIdx} $. While such undesirable behavior is also theoretically possible with finite constellations, we see from simulation results in Section \ref{sec:simulationResults} that the proposed algorithm performs better than its non-iterative counterpart when a finite constellation is used, thereby making iterative algorithms practically relevant for mitigating interference when superimposed pilots are employed.
\end{remark}
